Slow Feature Analysis as Variational Inference Objective

This work presents a novel probabilistic interpretation of Slow Feature Analysis (SFA) through the lens of variational inference. Unlike prior formulations that recover linear SFA from Gaussian state-space models with linear emissions, this approach relaxes the key constraint of linearity. While it does not lead to full equivalence to non-linear SFA, it recasts the classical slowness objective in a variational framework. Specifically, it allows the slowness objective to be interpreted as a regularizer to a reconstruction loss. Furthermore, we provide arguments, why -- from the perspective of slowness optimization -- the reconstruction loss takes on the role of the constraints that ensure informativeness in SFA. We conclude with a discussion of potential new research directions.

==> bdprocess.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}[scale=0.7, every node/.style={scale=0.7}, ->, node distance=1.75cm, state/.style={circle, draw, minimum size=1.2cm}]
  \node[state] (A)                    {$s_0$};
  \node[state]         (B) [right of=A] {$s_1$};
  \node[state, draw=blue!0] (dots) [right of=B] {$\dots$};
  \node[state]         (C) [right of=dots] {$s_{N-2}$};
  \node[state]         (D) [right of=C] {$s_{N-1}$};

  \draw[auto] 
        (A) edge [loop left]node {$1 - \theta$} (A)
        (A) edge [bend left] node {$\theta$} (B) 
        (B) edge [bend left] node {$1 - \theta$} (A)
        
        (B) edge [bend left] node {$\theta$} (dots)
        (dots) edge [bend left] node {$1 - \theta$} (B)
        
        (dots) edge [bend left] node {$\theta$} (C)
        (C) edge [bend left] node {$1 - \theta$} (dots)
        
        (C) edge [bend left] node {$\theta$} (D)
        (D) edge [bend left] node {$1 - \theta$} (C)
        
        (D) edge [loop right] node {$\theta$} (D);
\end{tikzpicture}
\caption{The schematic of a simple birth-death-process parameterized by a scalar $\theta$.}
    \label{fig:bd_graph}
\end{figure}

==> gdprocess.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}[scale=0.7, every node/.style={scale=0.7}, ->, node distance=2.5cm, state/.style={circle, draw, minimum size=1.2cm}]
  \node[state] (A)                    {$s_0$};
  \node[state]         (B) [right of=A] {$s_1$};
  \node[state, draw=blue!0] (dots) [right of=B] {$\dots$};
  \node[state]         (C) [right of=dots] {$s_{N-2}$};
  \node[state]         (D) [right of=C] {$s_{N-1}$};

  \draw[auto] 
        (A) edge [loop left]node {$1 - \theta$} (A)
        (A) edge [bend left] node {$\theta$} (B) 
        (B) edge [bend left] node {$1 - \theta$} (A)
        
        (B) edge [bend left] node {$\theta$} (dots)
        (dots) edge [bend left] node {$1 - \theta$} (B)
        
        (dots) edge [bend left] node {$\theta$} (C)
        (C) edge [bend left] node {$1 - \theta$} (dots)
        
        (C) edge [bend left] node {$\theta$} (D)
        (D) edge [bend left] node {$1 - \theta$} (C)
        
        (D) edge [loop right] node {$\theta$} (D);
\end{tikzpicture}
\caption{The schematic of a simplified and finite birth-death-process parameterized by a scalar $\theta$.}
    \label{fig:gd_graph}
\end{figure}

==> graphs/simple_model_with_var.tex <==
\setlength{\belowcaptionskip}{-8pt}
\begin{wrapfigure}{r}{0.2\textwidth}
\centering

\scalebox{0.8}{
\begin{tikzpicture}
  % Define nodes
  \node[obs, minimum size=\minnodesize]                               (x) {$\mathbf{x}$};
  \node[latent, above=of x, xshift=0cm, minimum size=\minnodesize] (z) {$\mathbf{z}$};
  \node[const, below=of x, inner sep=4pt] (theta) {$\theta$};
  \node[const, above=of z, inner sep=8pt, yshift=+10pt, color=\variationalcolor] (phi) {$\phi$};

  % Connect the nodes
  \edge {z, theta} {x} ; %
  \edge[dashed, \variationalcolor] {phi} {z};
  \path (x) edge [->, >={triangle 45}, dashed, \variationalcolor, bend right=45] (z);
\end{tikzpicture}
}
    \caption{Assumptions (generative and variational) in graphical model notation.}
    \label{fig:vaesfa_basic_model_with_var}
\end{wrapfigure}
\setlength{\belowcaptionskip}{0pt}

==> room_graph.tex <==
\setlength{\belowcaptionskip}{-12pt}
\begin{wrapfigure}{r}{0.4\textwidth}
\centering
 \begin{tikzpicture}[
            > = stealth, % arrow head style
            auto,
            node distance = 0.7cm, % distance between nodes
            semithick % line style
        ]

        \tikzstyle{every state}=[
            draw = black,
            thick,
            fill = white,
            minimum size = 4mm,
            scale=0.35
        ]
\node[state] (s0000) [] {};
\node[state] (s0100) [right of=s0000] {};
\node[state] (s0200) [right of=s0100] {};
\node[state] (s0300) [right of=s0200] {};
\node[state] (s0400) [right of=s0300] {};
\node[state] (s0500) [right of=s0400] {};
\node[state] (s0600) [right of=s0500] {};
\node[state] (s0700) [right of=s0600] {};
\node[state] (s0800) [right of=s0700] {};
\node[state] (s0900) [right of=s0800] {};
\node[state] (s0001) [below of=s0000] {};
\node[state] (s0101) [right of=s0001] {};
\node[state] (s0201) [right of=s0101] {};
\node[state] (s0301) [right of=s0201] {};
\node[state] (s0401) [right of=s0301] {};
\node[state] (s0501) [right of=s0401] {};
\node[state] (s0601) [right of=s0501] {};
\node[state] (s0701) [right of=s0601] {};
\node[state] (s0801) [right of=s0701] {};
\node[state] (s0901) [right of=s0801] {};
\node[state] (s0002) [below of=s0001] {};
\node[state] (s0102) [right of=s0002] {};
\node[state] (s0202) [right of=s0102] {};
\node[state] (s0302) [right of=s0202] {};
\node[state] (s0402) [right of=s0302] {};
\node[state] (s0502) [right of=s0402] {};
\node[state] (s0602) [right of=s0502] {};
\node[state] (s0702) [right of=s0602] {};
\node[state] (s0802) [right of=s0702] {};
\node[state] (s0902) [right of=s0802] {};
\node[state] (s0003) [below of=s0002] {};
\node[state] (s0103) [right of=s0003] {};
\node[state] (s0203) [right of=s0103] {};
\node[state] (s0303) [right of=s0203] {};
\node[state] (s0403) [right of=s0303] {};
\node[state] (s0503) [right of=s0403] {};
\node[state] (s0603) [right of=s0503] {};
\node[state] (s0703) [right of=s0603] {};
\node[state] (s0803) [right of=s0703] {};
\node[state] (s0903) [right of=s0803] {};
\node[state] (s0004) [below of=s0003] {};
\node[state] (s0104) [right of=s0004] {};
\node[state] (s0204) [right of=s0104] {};
\node[state] (s0304) [right of=s0204] {};
\node[state] (s0404) [right of=s0304] {};
\node[state] (s0504) [right of=s0404] {};
\node[state] (s0604) [right of=s0504] {};
\node[state] (s0704) [right of=s0604] {};
\node[state] (s0804) [right of=s0704] {};
\node[state] (s0904) [right of=s0804] {};
\node[state] (s0005) [below of=s0004] {};
\node[state] (s0105) [right of=s0005] {};
\node[state] (s0205) [right of=s0105] {};
\node[state] (s0305) [right of=s0205] {};
\node[state] (s0405) [right of=s0305] {};
\node[state] (s0505) [right of=s0405] {};
\node[state] (s0605) [right of=s0505] {};
\node[state] (s0705) [right of=s0605] {};
\node[state] (s0805) [right of=s0705] {};
\node[state] (s0905) [right of=s0805] {};
\node[state] (s0006) [below of=s0005] {};
\node[state] (s0106) [right of=s0006] {};
\node[state] (s0206) [right of=s0106] {};
\node[state] (s0306) [right of=s0206] {};
\node[state] (s0406) [right of=s0306] {};
\node[state] (s0506) [right of=s0406] {};
\node[state] (s0606) [right of=s0506] {};
\node[state] (s0706) [right of=s0606] {};
\node[state] (s0806) [right of=s0706] {};
\node[state] (s0906) [right of=s0806] {};
\node[state] (s0007) [below of=s0006] {};
\node[state] (s0107) [right of=s0007] {};
\node[state] (s0207) [right of=s0107] {};
\node[state] (s0307) [right of=s0207] {};
\node[state] (s0407) [right of=s0307] {};
\node[state] (s0507) [right of=s0407] {};
\node[state] (s0607) [right of=s0507] {};
\node[state] (s0707) [right of=s0607] {};
\node[state] (s0807) [right of=s0707] {};
\node[state] (s0907) [right of=s0807] {};
\node[state] (s0008) [below of=s0007] {};
\node[state] (s0108) [right of=s0008] {};
\node[state] (s0208) [right of=s0108] {};
\node[state] (s0308) [right of=s0208] {};
\node[state] (s0408) [right of=s0308] {};
\node[state] (s0508) [right of=s0408] {};
\node[state] (s0608) [right of=s0508] {};
\node[state] (s0708) [right of=s0608] {};
\node[state] (s0808) [right of=s0708] {};
\node[state] (s0908) [right of=s0808] {};
\node[state] (s0009) [below of=s0008] {};
\node[state] (s0109) [right of=s0009] {};
\node[state] (s0209) [right of=s0109] {};
\node[state] (s0309) [right of=s0209] {};
\node[state] (s0409) [right of=s0309] {};
\node[state] (s0509) [right of=s0409] {};
\node[state] (s0609) [right of=s0509] {};
\node[state] (s0709) [right of=s0609] {};
\node[state] (s0809) [right of=s0709] {};
\node[state] (s0909) [right of=s0809] {};

\path[-] (s0000) edge node {} (s0100);
\path[-] (s0100) edge node {} (s0200);
\path[-] (s0200) edge node {} (s0300);
\path[-] (s0300) edge node {} (s0400);
\path[-] (s0400) edge node {} (s0500);
\path[-] (s0500) edge node {} (s0600);
\path[-] (s0600) edge node {} (s0700);
\path[-] (s0700) edge node {} (s0800);
\path[-] (s0800) edge node {} (s0900);
\path[-] (s0000) edge node {} (s0001);
\path[-] (s0001) edge node {} (s0101);
\path[-] (s0100) edge node {} (s0101);
\path[-] (s0101) edge node {} (s0201);
\path[-] (s0200) edge node {} (s0201);
\path[-] (s0201) edge node {} (s0301);
\path[-] (s0300) edge node {} (s0301);
\path[-] (s0301) edge node {} (s0401);
\path[-] (s0400) edge node {} (s0401);
\path[-] (s0401) edge node {} (s0501);
\path[-] (s0500) edge node {} (s0501);
\path[-] (s0501) edge node {} (s0601);
\path[-] (s0600) edge node {} (s0601);
\path[-] (s0601) edge node {} (s0701);
\path[-] (s0700) edge node {} (s0701);
\path[-] (s0701) edge node {} (s0801);
\path[-] (s0800) edge node {} (s0801);
\path[-] (s0801) edge node {} (s0901);
\path[-] (s0900) edge node {} (s0901);
\path[-] (s0001) edge node {} (s0002);
\path[-] (s0002) edge node {} (s0102);
\path[-] (s0101) edge node {} (s0102);
\path[-] (s0102) edge node {} (s0202);
\path[-] (s0201) edge node {} (s0202);
\path[-] (s0202) edge node {} (s0302);
\path[-] (s0301) edge node {} (s0302);
\path[-] (s0302) edge node {} (s0402);
\path[-] (s0401) edge node {} (s0402);
\path[-] (s0402) edge node {} (s0502);
\path[-] (s0501) edge node {} (s0502);
\path[-] (s0502) edge node {} (s0602);
\path[-] (s0601) edge node {} (s0602);
\path[-] (s0602) edge node {} (s0702);
\path[-] (s0701) edge node {} (s0702);
\path[-] (s0702) edge node {} (s0802);
\path[-] (s0801) edge node {} (s0802);
\path[-] (s0802) edge node {} (s0902);
\path[-] (s0901) edge node {} (s0902);
\path[-] (s0002) edge node {} (s0003);
\path[-] (s0003) edge node {} (s0103);
\path[-] (s0102) edge node {} (s0103);
\path[-] (s0103) edge node {} (s0203);
\path[-] (s0202) edge node {} (s0203);
\path[-] (s0203) edge node {} (s0303);
\path[-] (s0302) edge node {} (s0303);
\path[-] (s0303) edge node {} (s0403);
\path[-] (s0402) edge node {} (s0403);
\path[-] (s0403) edge node {} (s0503);
\path[-] (s0502) edge node {} (s0503);
\path[-] (s0503) edge node {} (s0603);
\path[-] (s0602) edge node {} (s0603);
\path[-] (s0603) edge node {} (s0703);
\path[-] (s0702) edge node {} (s0703);
\path[-] (s0703) edge node {} (s0803);
\path[-] (s0802) edge node {} (s0803);
\path[-] (s0803) edge node {} (s0903);
\path[-] (s0902) edge node {} (s0903);
\path[-] (s0003) edge node {} (s0004);
\path[-] (s0004) edge node {} (s0104);
\path[-] (s0103) edge node {} (s0104);
\path[-] (s0104) edge node {} (s0204);
\path[-] (s0203) edge node {} (s0204);
\path[-] (s0204) edge node {} (s0304);
\path[-] (s0303) edge node {} (s0304);
\path[-] (s0304) edge node {} (s0404);
\path[-] (s0403) edge node {} (s0404);
\path[-] (s0404) edge node {} (s0504);
\path[-] (s0503) edge node {} (s0504);
\path[-] (s0504) edge node {} (s0604);
\path[-] (s0603) edge node {} (s0604);
\path[-] (s0604) edge node {} (s0704);
\path[-] (s0703) edge node {} (s0704);
\path[-] (s0704) edge node {} (s0804);
\path[-] (s0803) edge node {} (s0804);
\path[-] (s0804) edge node {} (s0904);
\path[-] (s0903) edge node {} (s0904);
\path[-] (s0004) edge node {} (s0005);
\path[-] (s0005) edge node {} (s0105);
\path[-] (s0104) edge node {} (s0105);
\path[-] (s0105) edge node {} (s0205);
\path[-] (s0204) edge node {} (s0205);
\path[-] (s0205) edge node {} (s0305);
\path[-] (s0304) edge node {} (s0305);
\path[-] (s0305) edge node {} (s0405);
\path[-] (s0404) edge node {} (s0405);
\path[-] (s0405) edge node {} (s0505);
\path[-] (s0504) edge node {} (s0505);
\path[-] (s0505) edge node {} (s0605);
\path[-] (s0604) edge node {} (s0605);
\path[-] (s0605) edge node {} (s0705);
\path[-] (s0704) edge node {} (s0705);
\path[-] (s0705) edge node {} (s0805);
\path[-] (s0804) edge node {} (s0805);
\path[-] (s0805) edge node {} (s0905);
\path[-] (s0904) edge node {} (s0905);
\path[-] (s0005) edge node {} (s0006);
\path[-] (s0006) edge node {} (s0106);
\path[-] (s0105) edge node {} (s0106);
\path[-] (s0106) edge node {} (s0206);
\path[-] (s0205) edge node {} (s0206);
\path[-] (s0206) edge node {} (s0306);
\path[-] (s0305) edge node {} (s0306);
\path[-] (s0306) edge node {} (s0406);
\path[-] (s0405) edge node {} (s0406);
\path[-] (s0406) edge node {} (s0506);
\path[-] (s0505) edge node {} (s0506);
\path[-] (s0506) edge node {} (s0606);
\path[-] (s0605) edge node {} (s0606);
\path[-] (s0606) edge node {} (s0706);
\path[-] (s0705) edge node {} (s0706);
\path[-] (s0706) edge node {} (s0806);
\path[-] (s0805) edge node {} (s0806);
\path[-] (s0806) edge node {} (s0906);
\path[-] (s0905) edge node {} (s0906);
\path[-] (s0006) edge node {} (s0007);
\path[-] (s0007) edge node {} (s0107);
\path[-] (s0106) edge node {} (s0107);
\path[-] (s0107) edge node {} (s0207);
\path[-] (s0206) edge node {} (s0207);
\path[-] (s0207) edge node {} (s0307);
\path[-] (s0306) edge node {} (s0307);
\path[-] (s0307) edge node {} (s0407);
\path[-] (s0406) edge node {} (s0407);
\path[-] (s0407) edge node {} (s0507);
\path[-] (s0506) edge node {} (s0507);
\path[-] (s0507) edge node {} (s0607);
\path[-] (s0606) edge node {} (s0607);
\path[-] (s0607) edge node {} (s0707);
\path[-] (s0706) edge node {} (s0707);
\path[-] (s0707) edge node {} (s0807);
\path[-] (s0806) edge node {} (s0807);
\path[-] (s0807) edge node {} (s0907);
\path[-] (s0906) edge node {} (s0907);
\path[-] (s0007) edge node {} (s0008);
\path[-] (s0008) edge node {} (s0108);
\path[-] (s0107) edge node {} (s0108);
\path[-] (s0108) edge node {} (s0208);
\path[-] (s0207) edge node {} (s0208);
\path[-] (s0208) edge node {} (s0308);
\path[-] (s0307) edge node {} (s0308);
\path[-] (s0308) edge node {} (s0408);
\path[-] (s0407) edge node {} (s0408);
\path[-] (s0408) edge node {} (s0508);
\path[-] (s0507) edge node {} (s0508);
\path[-] (s0508) edge node {} (s0608);
\path[-] (s0607) edge node {} (s0608);
\path[-] (s0608) edge node {} (s0708);
\path[-] (s0707) edge node {} (s0708);
\path[-] (s0708) edge node {} (s0808);
\path[-] (s0807) edge node {} (s0808);
\path[-] (s0808) edge node {} (s0908);
\path[-] (s0907) edge node {} (s0908);
\path[-] (s0008) edge node {} (s0009);
\path[-] (s0009) edge node {} (s0109);
\path[-] (s0108) edge node {} (s0109);
\path[-] (s0109) edge node {} (s0209);
\path[-] (s0208) edge node {} (s0209);
\path[-] (s0209) edge node {} (s0309);
\path[-] (s0308) edge node {} (s0309);
\path[-] (s0309) edge node {} (s0409);
\path[-] (s0408) edge node {} (s0409);
\path[-] (s0409) edge node {} (s0509);
\path[-] (s0508) edge node {} (s0509);
\path[-] (s0509) edge node {} (s0609);
\path[-] (s0608) edge node {} (s0609);
\path[-] (s0609) edge node {} (s0709);
\path[-] (s0708) edge node {} (s0709);
\path[-] (s0709) edge node {} (s0809);
\path[-] (s0808) edge node {} (s0809);
\path[-] (s0809) edge node {} (s0909);
\path[-] (s0908) edge node {} (s0909);
    \end{tikzpicture}
    \caption{Example of a lattice with $10\times10$ states}
    \label{fig:single_room_graph}
\end{wrapfigure}
\setlength{\belowcaptionskip}{0pt}
%The single room environment used for analysing optimal embeddings. 


